Contention-Aware GPU Partitioning and Task-to-Partition Allocation for Real-Time Workloads

In order to satisfy timing constraints, modern real-time applications require massively parallel accelerators such as General Purpose Graphic Processing Units (GPGPUs). Generation after generation, the number of computing clusters made available in novel GPU architectures is steadily increasing, hence, investigating suitable scheduling approaches is now mandatory. Such scheduling approaches are related to mapping different and concurrent compute kernels within the GPU computing clusters, hence grouping GPU computing clusters into schedulable partitions. In this paper we propose novel techniques to define GPU partitions; this allows us to define suitable task-to-partition allocation mechanisms in which tasks are GPU compute kernels featuring different timing requirements. Such mechanisms will take into account the interference that GPU kernels experience when running in overlapping time windows. Hence, an effective and simple way to quantify the magnitude of such interference is also presented. We demonstrate the efficiency of the proposed approaches against the classical techniques that considered the GPU as a single, non-partitionable resource.

==> texfiles/shepherd.tex <==
 ----------------------- REVIEW 1 ---------------------
SUBMISSION: 35
TITLE: Contention-Aware GPU Partitioning and Task-to-Partition Allocation for Real-Time Workloads
AUTHORS: Zahaf Houssam-Eddine, Sanudo Olmedo Ignacio, Singh Jayati, Capodieci Nicola and Faucou Sebastien

----------- Overview of the paper's contributions -----------
The paper proposes a GPU partitioning and task-to-partition assignment heuristics. The technique takes into account the resource contention. The authors study the performance of the heuristics in comparison with the state of the art.
----------- Overall evaluation -----------
The authors are studying a problem relevant to our community, the work is well motivated.

I regret that the document is difficult to follow for a reader interested in modern architectures, their programming and related scheduling issues. Indeed, the document is not accessible without a fairly deep knowledge of how to program on the target architect (here NVIDIA). The authors do not give enough information to the readers, the document is, according to my level of expertise, too technical, not conceptual enough. Moreover, one can doubt the genericness of the proposed technique and performance.

Detailed comments

An introduction to NVIDIA architecture, programming paradigm (with illustrations) is missing.

Undefined terms: OEM, compute kernels, GPU compute resources, processes, GPGPU, GPU kernels (equivalent to compute kernels?), compute grid, GPU partition

Unclear concepts: streaming multiprocessors, Multi-process service, Multi-Instance GPU, GPU kernel, blocks, thread, warp.

Figure 2 and equation C(m): what we learn here?, from my understanding this is a consequence of the Amdahl's law?

The dichotomy between compute intensive and memory intensive seems simplistic to me, can we consider an additional parameter as a percentage?

Regarding the experiments, from my understanding the simulation duration is the hyper-period. I'm wondering if this is significant, if the first hyper-period corresponds to the worst-case or to the periodic behaviour of the system?


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 ----------------------- REVIEW 2 ---------------------
SUBMISSION: 35
TITLE: Contention-Aware GPU Partitioning and Task-to-Partition Allocation for Real-Time Workloads
AUTHORS: Zahaf Houssam-Eddine, Sanudo Olmedo Ignacio, Singh Jayati, Capodieci Nicola and Faucou Sebastien

----------- Overview of the paper's contributions -----------
This paper presents a heuristic for partitioning a shared GPU among a task system, generating partition assignments and sizes.
----------- Overall evaluation -----------
This paper describes a mechanism for partitioning GPU resources, depending on
tasks' resource requirements.  The heuristic gradually merges partitions until
a task system is schedulable, i.e. it fits in the GPU's resource requirements
and all tasks have sufficient resources to meet their deadlines.  The desire
for GPU partitioning has long been a feature of real-time research, and the
partitioning heuristic is not particularly surprising, but the paper still
makes a contribution and seems to be a good fit for RTNS.

There is one primary weakness to the paper's approach, however.  The proposed
heuristic (and overall SM-based approach to partitioning) is unlikely to
correspond to hardware capabilities of real GPUs.  Specifically, the paper
mentions NVIDIA's MIG (Multi-instance GPU) in Section 1.  MIG is likely (I have
yet to use it) a far better GPU-sharing approach than MPS, but the current MIG
documentation indicates that partitions will be limited to power-of-two
divisions of the GPU's resources, rather than an arbitrary list of SMs.  The
paper's heuristic instead assumes finer-grained control over individual SMs
(Section 4.1).  This may be possible with current software-based techniques
from prior work, but the software-based techniques wouldn't provide the memory
isolation expected elsewhere in the paper.  In short, to apply on real hardware
the paper's heuristic would either need to be changed to use MIG's partitioning
model, or to use some other mechanism for memory isolation.

Probably because of this weakness, the experiments consider only synthetic
task systems and not real GPU workloads.

There are a few parts of the heuristic that are unclear in the text:

 - What is the meaning of "fill_forbidden_list" on line 3 of Algorithm 1? It
   doesn't seem to be referenced or defined elsewhere in the text or algorithm.

 - The sentence after Lemma 1 starting "Therefore, when a task executes on all
   resources..." is hard to understand.

 - Near the start of 5.1, it is unclear what is meant by "no concurrency" in
   "As the task executes with no concurrency..." Perhaps "without contending
   with other tasks" would be better than "with no concurrency?"

 - Near the start of 5.2, what is meant by "optimal" in "Even if the number of
   required SMs per partition is optimal, ..."?

 - In Algorithm 2, line 3, shouldn't the second P^1 in T(P^1 \oplus P^1) be P^2
   instead?

 - The text following Definition 3 and Definition 4 both states "We define
   partial relation order >> as follows". However, Definition 4 seems like it
   should read "... partial relation order > as follows..."

 - In Algorithm 3 (and the related text) why abbreviate "eligible" as "elli"?
   (i.e. "elli_list") Perhaps use "elig_list" instead?

 - It would be nice if the line styles for "Worst" and "Best" were the same in
   Figures 5 and 7.

Other small things:

Spell out "OEM" in the intro.

The use of the word "compound" in Section 4.1 is strange.

In Section 4.2, add a formal definition of "conflict".

In Section 5.2, please say explitcitly what you mean by "tail effect".

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 ----------------------- REVIEW 3 ---------------------
SUBMISSION: 35
TITLE: Contention-Aware GPU Partitioning and Task-to-Partition Allocation for Real-Time Workloads
AUTHORS: Zahaf Houssam-Eddine, Sanudo Olmedo Ignacio, Singh Jayati, Capodieci Nicola and Faucou Sebastien

----------- Overview of the paper's contributions -----------
This paper presents a novel GPU partitioning and allocation method that, unlike other methods in the literature, can meet task deadline requirements. The method involves partitioning of SMs (Streaming Multiprocessors), and then allocate kernel tasks into the partitions. In the evaluation the proposed method is compared with the baseline which is the case that GPU is not shared.

Overall the paper is well written and is easy to follow. The research topic also meets the expectation of RTNS. However there are some missing points that need to be further addressed, which will be discussed below. Hence, I suggest a (weak) acceptance.
----------- Overall evaluation -----------
## Major comments
- The task model is too simplified. First in the conflicted case, it is not so obvious how would the worst-case execution time be affected by the interference, e.g., shared cache. It also provides no insight how would this C_i in conflict case can be obtained.
- After Lemma 1, "The task execution time never increases with the increase of the number of resources" --- this is more an assumption than a statement. In some anomaly cases, this can be invalid due to the overhead of copying data to "fork" a new parallel branch.
- The definition of memory intensive and compute intensive need to be more elaborated. First a binary classification is oversimplified; Second in the experiment, prm is fixed to 50% which brings the question -- would the result be different if this value is different? This may need more experiment or discussion.
- Even the problem of interested is NP-hard, it is still important to give some insights of the optimally of the heuristic in some way, e.g., comparing with an exhaustive or meta-heuristic (for example, GA) search.

-

## Minor issues
- In Figure 3, put the exact numbers on top of the bar charts to make the diagram more informative.
- In Section 5.1, "As the task executes with no concurrency" -- this is not precise as within a SM the thread will be executed concurrently.
- Algorithm 2, the notation P1 and P2 should be P^1 and P^2.
- Definition 4, '>>' should be '>'.
- The forbidden list (Section 5.3) needs more explanation, especially how it is initialized.
- For Figure 5 and Figure 7, the legends need to either be more distinguishable or use a different color.



==> texfiles/tmp.tex <==



\paragraph{Example.}
\he{The example need to be revised to fullfill with the new model}

Let $\tau$ be a task compound of $5$ blocks. The task period is set to
$20$, and a deadline of $7$. A block executes for $1$ time unit, if
executed with a memory intensive kernel, and $2$ time units when
allocated with a compute intensive kernel. 



Let consider first that all blocks of the task are allocated to
partition $p_1$. In Figure \ref{fig:task:example}, they have a red
color. The task is allocated with a memory intensive kernel, colored
in blue. Therefore, every task block has an execution time that equals
to $1$, and the task execution time is set to $5$. On the right part
of the figure, the task blocks are allocated to $p 1$ and to
$p_2$. For parition $p_1$, $3$ blocks of the task are allocated with a
memory intensive task, therefore their execution time is set to 1. On
the second partition, task blocks are allocated with a compute kernel,
therefore, block execution time is equal to $2$. As two blocks are
allocated to partition $p_2$, the task execution time on partition
$p_2$, is equal to $\mathsf{WCET}(\tau,p_2)=4$.

\begin{figure}[h]
  \centering
  \resizebox{0.45\textwidth}{!}{
  \begin{tikzpicture}

\foreach \x in {1,2,...,5}
{
\draw (0, \x -0.2) -- (7, \x-0.2); 
\draw[draw=black, fill=red!40, opacity=0.3] (\x-1,1.2) rectangle  (\x,0.8);
\draw[->] (0, \x-0.2) --(0,\x+0.7); 

\node at (-0.8, \x+0.25){\sf p \x};
}


\def\y{1}
\foreach \x in {0,1.4,...,5}
{

\draw[draw=black, fill=blue!40, opacity=0.3] (\x,1.2) rectangle  (\x+1.4,1.6);
\def\y{\x+0.4}
}


\draw [dashed] (0,1) --(0, 0);
\draw [dashed] (5,1) --(5, 0);




\draw [<->] (0,-0.2) -- (5,-0.2);
\draw[fill=white,draw=white ] (1.8, -0.5) rectangle (3.2,0.1);
\node at (2.5, -0.2) {\small \sf WCET}; 


\draw [dashed] (1,1) --(1, 0.4);
\draw [dashed] (2,1) --(2, 0.4);

\draw[fill=white, draw=white] (1.3, 0.6) rectangle (1.8,0.1);
\draw [<->] (1,0.5) -- (2,0.5);
\draw[fill=white, draw=white] (1.3, 0.6) rectangle (1.8,0.1);

\node at (1.5, 0.4) {\tiny $\mathcal{C}_j^{M}$}; 


\end{tikzpicture}}\quad
\resizebox{0.45\textwidth}{!}{\begin{tikzpicture}
\foreach \x in {1,2,...,5}
{
\draw (0, \x -0.2) -- (7, \x-0.2); 
\draw[->] (0, \x-0.2) --(0,\x+0.7); 
\node at (-0.8, \x+0.25){\sf p \x};
}


\foreach \x in {1,2,...,3}
{
\draw (0, \x -0.2) -- (7, \x-0.2); 
\draw[draw=black, fill=red!40, opacity=0.3] (\x-1,1.2) rectangle  (\x,0.8);
\draw[->] (0, \x-0.2) --(0,\x+0.7); 
\node at (-0.8, \x+0.25){\sf p \x};
}


\def\y{1}
\foreach \x in {0,1.4,...,5}
{
\draw[draw=black, fill=blue!40, opacity=0.3] (\x,1.2) rectangle  (\x+1.4,1.6);
\def\y{\x+0.4}
}
\draw [dashed] (0,1) --(0, 0);
\draw [dashed] (4,2) --(4, 0);
\draw [<->] (0,-0.2) -- (4,-0.2);
\draw[fill=white, ,draw=white ] (1.4, -0.5) rectangle (2.6,0.1);
\node at (2, -0.2) {\small \sf WCET}; 
\draw [dashed] (1,1) --(1, 0.4);
\draw [dashed] (2,1) --(2, 0.4);
\draw[fill=white, draw=white] (1.3, 0.6) rectangle (1.8,0.1);
\draw [<->] (1,0.5) -- (2,0.5);
\draw[fill=white, draw=white] (1.3, 0.6) rectangle (1.8,0.1);

\node at (1.5, 0.4) {\tiny $\mathcal{C}_j^{C}$}; 

\foreach \x in {0,2,...,2}
{
\draw [fill=red!40, opacity=0.4](\x,1.8) rectangle (\x+2,2.2); 
}


\foreach \x in {0,2.5,...,4}
{
\draw [fill=green!40, opacity=0.4](\x,2.2) rectangle (\x+2.5,2.6); 
}


\end{tikzpicture}} 
  \caption{Example of a task }
  \label{fig:task:example}
\end{figure}


